An Investigation of Noise in Morphological Inflection

With a growing focus on morphological inflection systems for languages where high-quality data is scarce, training data noise is a serious but so far largely ignored concern. We aim at closing this gap by investigating the types of noise encountered within a pipeline for truly unsupervised morphological paradigm completion and its impact on morphological inflection systems: First, we propose an error taxonomy and annotation pipeline for inflection training data. Then, we compare the effect of different types of noise on multiple state-of-the-art inflection models. Finally, we propose a novel character-level masked language modeling (CMLM) pretraining objective and explore its impact on the models' resistance to noise. Our experiments show that various architectures are impacted differently by separate types of noise, but encoder-decoders tend to be more robust to noise than models trained with a copy bias. CMLM pretraining helps transformers, but has lower impact on LSTMs.

==> annotation_section_old.tex <==
We develop an automated pipeline to annotate each inflection pair from a taxonomy of noise, primarily relying on rule-based morphological analyzers for each language from Apertium. Here we describe each type of noise in our taxonomy. For a description of how each type of noise is detected, see Section \cref{sec:appendix_detecting_noise} in the appendix.

\paragraph{Lexicon Noise}
Any word type that is not in the standard vocabulary 
of a given language is considered lexicon noise.

% \paragraph{Detection} 
% We use three resources to form the lexicon of each language: Apertium, Wikipedia, and a python spellchecker\footnote{\href{https://github.com/dvwright/phunspell}{https://github.com/dvwright/phunspell}} based on hunspell\footnote{\href{http://hunspell.github.io/}{http://hunspell.github.io/}}. Any word not in any of these three is lexicon noise.
We expect this noise to come from archaisms, borrowings, and biblical references. This means that lexicon noise \textit{could} follow the regular inflections of a language, and in that case may have a low impact on downstream inflection systems. It could also have a positive impact by increasing training data size, likely with higher lemma diversity. However, lexicon noise could also entail archaic or borrowed \textit{inflections}, which would introduce non-existent transformations. In general, lexicon noise could also occur due to language, dialect, or orthography mixing -- though we expect this to be somewhat rare in the bible corpora that we build upon.

\begin{figure}[t]
     \centering
     \includegraphics[width=0.55\linewidth]{figs/stacked_noise_by_lang.pdf}
    \caption{tUMPC noise distribution for all languages.}
    \label{fig:baseline_noise}
\end{figure}

\paragraph{POS Noise}
Not all parts of speech inflect, and this varies by language. However, tUMPC sometimes induces spurious inflection pairs from words that do not inflect, like conjunctions or prepositions in most languages. Any word of a POS that does not inflect in the given language is thus considered POS noise. 
This is detected with the Apertium POS,
 
but ultimately these samples will be assigned an MSD 
 from UniMorph with a POS that does inflect.
% \paragraph{Detection}
% Here we produce lists of POS that inflect for each language. Any word whose Apertium analysis does not contain any valid POS according to this list is considered POS noise. For details on the valid POS, see Table \ref{tab:appendix_valid_pos} in the appendix.

While inflection pairs with POS noise may sometimes have real transformations, it is highly likely that these add spurious inflections to the training data. For this reason, we expect POS noise to consistently cause mistakes in each system.

\paragraph{POS Pair Noise}
Two words from different POS forming an inflection pair constitutes POS pair noise. This can occur when tUMPC puts two completely unrelated words in the same paradigm, but this could also arise due to valid derivations. The latter case could be considered a morphological transformation that our model should learn. There is debate around whether or not there is a clearly defined distinction between inflection and derivation \cite{haspelmathinflection},
but since our goal is to evaluate on SIGMORPHON shared task data that does not include derivation, we consider this noise in our pipeline. 

POS pair noise should have a similar impact as POS noise, except that due to derivations we expect several of the induced transformations to appear much more commonly in languages where productive derivation is pervasive. 
% AW: REMOVED -- Not really related to noisy training data, more to the source of a potential mistake in tUMPC
% Because derivation can cause two words from different lexemes to appear as if they are part of the same inflectional paradigm, the tUMPC pipeline might not only induce extra inflectional transformations, but also potentially unique paradigm slots corresponding to derivational patterns. 

\paragraph{Paradigm Noise}
Pairs of forms that do not belong to the same paradigm, but share a POS constitute paradigm noise. An example in English is $
\textrm{warp} ~ \rightarrow ~ 
\textrm{wraps} \nonumber$, where \textit{wraps} 
comes from a different paradigm than \textit{warp}.
% \paragraph{Detection}
% For a given inflection pair, if both words have no overlapping lemmas of the same POS (but \textit{do} have a shared POS) according to Apertium, we consider them to be from separate paradigms, and thus paradigm noise.
Because paradigm noise should contain target words expressing a valid inflection, it is possible that it will not have much negative impact on an inflection system's decoder. However, since paradigm noise also contains source forms that the target is not actually inflected from, the full transformation from source to target has the potential to be spurious. For example, in the $\textrm{warp} ~ \rightarrow ~ \textrm{wraps}$ example above, consider the apparent \textit{a, r} metathesis. This could cause models relying on a bias towards transduction to struggle more with paradigm noise than models relying predominantly on a decoder.

\paragraph{Slot Noise}
When the target word in an inflection pair has an incorrect MSD, we mark this as slot noise. For example, consider an inflection $
\textrm{cry} ~ \rightarrow ~ 
\textrm{cried} \nonumber$, which is a valid inflection pair, but if, for example, \textit{cried} is incorrectly marked as the third person present, this would be slot noise. Our training setup makes use of \textit{only} the target slot -- if only the source form has an incorrect slot then a pair is not marked as slot noise.
% \paragraph{Detection}
% Slot noise occurs when the slot assigned to a word by tUMPC is not in the set of slots from Apertium analysis. We rely on the version of tUMPC and Apertium slots that have been mapped to UniMorph for this part of the annotation. Slot noise considers only the predicted and gold MSD for a slot, so it can can co-occur on a single sample with any other noise in the taxonomy.
% This requires a mapping from Apertium morphological tags to tUMPC slot identifiers. Because our downstream evaluation is on the SIGMORPHON development sets, we align each word's slot to the UniMorph MSDs used in the SIGMORPHON data in practice. We give more detail on these mappings in the next subsection.
This error results in a mismatch of MSDs and inflectional transformations. So, for some paradigms, the output form for an inflection can be thought of as swapped with another output form in the same paradigm. If these two forms are different, this is likely to confuse the inflection system by presenting counter-evidence to the correct inflection. Additionally, it is possible that there are few to no correctly tagged instances of rare or irregular inflection classes, causing a system to confidently learn that, e.g., the past tense inflection is the third person present.
